Two-Level Temporal Relation Model for Online Video Instance Segmentation

In Video Instance Segmentation (VIS), current approaches either focus on the quality of the results, by taking the whole video as input and processing it offline; or on speed, by handling it frame by frame at the cost of competitive performance. In this work, we propose an online method that is on par with the performance of the offline counterparts. We introduce a message-passing graph neural network that encodes objects and relates them through time. We additionally propose a novel module to fuse features from the feature pyramid network with residual connections. Our model, trained end-to-end, achieves state-of-the-art performance on the YouTube-VIS dataset within the online methods. Further experiments on DAVIS demonstrate the generalization capability of our model to the video object segmentation task. Code is available at: \url{https://github.com/caganselim/TLTM}

==> sec/cmd.tex <==
\usepackage{shdoc}
\usepackage{tabulary,overpic,xcolor}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{float}

\definecolor{mygray}{gray}{.92}
\definecolor{myred}{rgb}{1,0.5,0.5}
\definecolor{myred2}{rgb}{0.75,0,0}

% Typeset vectors in bold
\newcommand{\vc}[1]{\boldsymbol{#1}}
\newcommand{\vb}[1]{\mathbf{#1}}
\newcommand{\bd}[1]{\textbf{#1}}

\usepackage{float}
\usepackage{tikz}
\usepackage{mathrsfs}
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 

